The Importance of Downstream Networks in Digital Pathology Foundation Models

Digital pathology has significantly advanced disease detection and pathologist efficiency through the analysis of gigapixel whole-slide images (WSI). In this process, WSIs are first divided into patches, for which a feature extractor model is applied to obtain feature vectors, which are subsequently processed by an aggregation model to predict the respective WSI label. With the rapid evolution of representation learning, numerous new feature extractor models, often termed foundational models, have emerged. Traditional evaluation methods rely on a static downstream aggregation model setup, encompassing a fixed architecture and hyperparameters, a practice we identify as potentially biasing the results. Our study uncovers a sensitivity of feature extractor models towards aggregation model configurations, indicating that performance comparability can be skewed based on the chosen configurations. By accounting for this sensitivity, we find that the performance of many current feature extractor models is notably similar. We support this insight by evaluating seven feature extractor models across three different datasets with 162 different aggregation model configurations. This comprehensive approach provides a more nuanced understanding of the feature extractors' sensitivity to various aggregation model configurations, leading to a fairer and more accurate assessment of new foundation models in digital pathology.

==> tables/tab1_transposed.tex <==
\begin{table*}[]
\caption{Feature model extraction details.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                                                                                & \textbf{Dino v2 (DP)}                                                                                                 & \textbf{Dino v2 (Natural)}                                                           & \textbf{iBOT} & \textbf{CTransPath}  & \textbf{REMEDIS}     & \textbf{BYOL (Ex Domain)}                                                                                              & \textbf{BYOL (In Domain)}                                                                                           \\ \hline
\textbf{Learning Approach}                                                      & Combination                                                                                                           & Combination                                                                          & Combination   & Contrastive Learning & Contrastive Learning & Non-Contrastive Learning                                                                                               & Non-Contrastive Learning                                                                                            \\ \hline
\textbf{Model Details}                                                          & ViT-L/14                                                                                                              & ViT-L/14 distilled                                                                   & ViT-B         & Swin Transformer     & BiT-M (ResNet-152x2) & ResNet50 (or 18?)                                                                                                      & ResNet50 (or 18?)                                                                                                   \\ \hline
\textbf{Model Size (Mio.)}                                                      & 300                                                                                                                   & 300                                                                                  & 86            & 280                  & 240                  & 26                                                                                                                     & 26                                                                                                                  \\ \hline
\textbf{Embedding Size}                                                         & 1024                                                                                                                  & 1024                                                                                 & 768           & 768                  & 4096                 & 2048                                                                                                                   & 2048                                                                                                                \\ \hline
\textbf{Dataset Content}                                                        & \begin{tabular}[c]{@{}c@{}}TCGA,\\ in-house data\\ (incl. clinical diverse\\  trial data and others) (?)\end{tabular} & \begin{tabular}[c]{@{}c@{}}LVD-142M\\ (incl. ImageNet-22k\\ and others)\end{tabular} & TCGA          & TCGA + PAIP          & TCGA                 & \begin{tabular}[c]{@{}c@{}}TCGA,\\ selected in-house data\\ (incl. clinical trial data\\  and others) (?)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Goya (clinical trial),\\ Cavalli (clinical trial),\\ Herohe, Camelyon16 (?)\end{tabular} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Dataset Size / \\ Tiles (Mio.)\end{tabular}} & 35                                                                                                                    & 142                                                                                  & 43            & 16                   & 50                   & 2 (?)                                                                                                                  & 2 (?)                                                                                                               \\ \hline
\textbf{Trained by Us (?)}                                                      & yes                                                                                                                   & no                                                                                   & no            & no                   & no                   & yes                                                                                                                    & yes                                                                                                                 \\ \hline
\end{tabular}
}
\end{table*}
